F$^{2}$-NeRF: Fast Neural Radiance Field Training with Free Camera Trajectories

This paper presents a novel grid-based NeRF called F2-NeRF (Fast-Free-NeRF) for novel view synthesis, which enables arbitrary input camera trajectories and only costs a few minutes for training. Existing fast grid-based NeRF training frameworks, like Instant-NGP, Plenoxels, DVGO, or TensoRF, are mainly designed for bounded scenes and rely on space warping to handle unbounded scenes. Existing two widely-used space-warping methods are only designed for the forward-facing trajectory or the 360-degree object-centric trajectory but cannot process arbitrary trajectories. In this paper, we delve deep into the mechanism of space warping to handle unbounded scenes. Based on our analysis, we further propose a novel space-warping method called perspective warping, which allows us to handle arbitrary trajectories in the grid-based NeRF framework. Extensive experiments demonstrate that F2-NeRF is able to use the same perspective warping to render high-quality images on two standard datasets and a new free trajectory dataset collected by us. Project page: https://totoro97.github.io/projects/f2-nerf.

==> figures/intro_trajectory.tex <==
\begin{figure}[htb]
  \includegraphics[width=\linewidth]{figure_resources/intro_trajectory} \caption{{\bf The pre-defined} camera capture patterns.}
  \label{fig:intro_trjectory}
\end{figure}


==> figures/rebuttal_longer.tex <==
\begin{figure}[htb]
  \includegraphics[width=\linewidth]{figure_resources/rebuttal_longer.pdf} \caption{Visual comparison on the ``Lab'' case of Free dataset.}
  \label{fig:rebuttal_longer}
\end{figure}


==> figures/supp_impl_lin_matrix.tex <==
\begin{figure}[htb]
  \includegraphics[width=\linewidth]{figure_resources/supp_impl_lin_matrix.pdf} \caption{{\bf Visual comparison between using rand matrix~(a) and using PCA matrix~(b).}}
  \label{fig:lin_matrix}
\end{figure}


==> tables/rebuttal_longer.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{@{}l@{\hskip 3pt}|@{\hskip 3pt}c@{\hskip 8pt}c@{\hskip 8pt}c@{\hskip 8pt}c@{}}
    \hline
    Method & Tr. time & PSNR{\scriptsize$\uparrow$} & SSIM{\scriptsize$\uparrow$} & LPIPS{\scriptsize(VGG)$\downarrow$} \\
    \hline\hline
    {\small F$^2$-NeRF$_{\rm 50k}$} & 33m & 26.69 & 0.775 & 0.292 \\
    {\small F$^2$-NeRF$_{\rm 100k}$} & 62m & 26.96 & 0.803 & 0.251 \\
    {\small F$^2$-NeRF$_{\rm 100k-large}$} & 70m & 27.42 & 0.831 & 0.211 \\
    \hline
    {\small mip-NeRF-360$_{\rm 500k}$} & 31h & 27.01 & 0.766 & 0.295  \\
    \hline
    \end{tabular}
    \vspace{-1em}
    \caption[]{Training F$^2$-NeRF for longer time on the Free dataset.}
    \label{tab:rubuttal_longer}
\end{table}

